Minimal Assumptions Refinement for GR(1) Specifications

Reactive synthesis is concerned with finding a correct-by-construction controller from formal specifications, typically expressed in Linear Temporal Logic (LTL). The specifications describe assumptions about an environment and guarantees to be achieved by the controller operating in that environment. If a controller exists, given the assumptions, the specification is said to be realizable. This paper focuses on finding a minimal set of assumptions that guarantee realizability in the context of counterstrategy-guided assumption refinement procedures. Specifically, we introduce the notion of minimal assumptions refinements and provide an algorithm that provably computes these with little time overhead. We show experimentally, using common benchmarks, that embedding our algorithm in state-of-the-art approaches for assumption refinement results in consistently shorter solutions than without such embedding, and allows to explore a higher number of candidate solutions. We also propose a hybrid variant for dealing with the higher sparsity of solutions in the space of minimal refinements and show that its application speeds up the identification of a solution.

==> sections/background.tex <==
\section{Background}
\label{sec:Background}
In the following we describe the basic syntax of the GR(1) specification language, give a formal definition of counterstrategy, and define the problem of assumptions refinement.

\subsection{LTL and GR(1)}
\label{sec:LTLGR1}
\emph{Linear temporal logic} (LTL) is an extension of propositional logic used in software engineering for describing requirements of systems \cite{Dwyer1999a,VanLamsweerde1998c,Manna1992}. %It extends propositional logic with operators that express properties of infinite sequences of assignments to Boolean variables, which model system executions over discrete time. Specifically, the extension involves the temporal operators $\next$ (``next''), which denotes that a subformula holds for the next step of the execution, $\until$ (``until''), which expresses that its first operand holds until its second operand holds, $\eventually$ (``eventually''/``finally''), which denotes that its operand holds at some point in the execution, $\always$ (``always''/``globally''), denoting that its operand must hold at every step in the execution.
Let $\var$ be a set of Boolean variables, and $\Sigma = 2^\var$ the set of all possible assignments/valuations to $\var$. We denote by $\Sigma^\omega$ the set of infinite sequences of elements in $\Sigma$, and for every $\pi \in \Sigma^\omega$ we denote by $\pi_i$ the $i-th$ element of the sequence. An LTL formula is an expression $\phi$ defined by the grammar (in Backus-Naur form)
$$\phi ::= p \:|\: \lnot \phi \:|\: \phi \land \phi \:|\: \next \phi \:|\: \phi \until \phi \;.$$
where $p \in \var$.
We say that a sequence $\pi \in \Sigma^\omega$ \emph{satisfies} $\phi$ (in symbols $\pi \models \phi$) if and only if one the following holds: (1) $\phi = p$ and $p \in \pi_1$, (2) $\phi = \lnot \phi'$ and $\pi \not\models \phi'$, (3) $\phi = \phi_1 \land \phi_2$ and $\pi \models \phi_1, \pi \models \phi_2$, (4) $\phi = \next \phi'$ and $\pi' = \pi_2\pi_3\dots \models \phi'$, (5) $\phi = \phi_1 \until \phi_2$, and there exists an index $k$ such that $\pi_k\pi_{k+1}\dots \models \phi_2$ and for every $i < k$ $\pi_i\pi_{i+1}\dots \models \phi_1$. The other Boolean operators ($\lor$, $\rightarrow$, $\leftrightarrow$) are defined as usual by using (1) and (2). The minimal set of temporal operators is extended with $\eventually \phi \equiv \true \until \phi$ and $\always \phi \equiv \lnot \eventually \lnot \phi$.

In this context we are interested in a subset of LTL called \emph{Generalized Reactivity (1)} \cite{Li2011b}. This includes formulae of the kind $\phi^\env \rightarrow \phi^\sys$, where both $\phi^\env$ and $\phi^\sys$ are conjunctions of three kinds of LTL formulae: (1) \emph{initial conditions}, purely Boolean formulae $\boolexprvar$ over the variables in $\var$ not containing any temporal operator, constraining the initial state of a system; (2) \emph{invariants}, of the form $\always \boolexpression(\var \cup \next\var)$, temporal formulae containing only an outer $\always$ operator and $\next$ operators such that no two $\next$ are nested; these formulae encode one-step transitions allowed in the system; (3) \emph{fairness conditions} of the form $\always\eventually \boolexprvar$, expressing a Boolean condition $\boolexprvar$ holding infinitely many times in a system execution. Each conjunct in $\phi^\env$ is called \emph{assumption}, and each one in $\phi^\sys$ is called \emph{guarantee}.

\subsection{GR(1) Games and Counterstrategies}
GR(1) formulae express properties of two-agent systems, where one of the agents is called \emph{environment} and the other \emph{controller}. The environment's state is characterized by a subset of variables $\inx \in \var$ called \emph{input variables}, while the controller's state is determined by the complementary subset $\outy = \var \setminus \inx$ of \emph{output variables}. The two agents compete in a game. Game states are valuations of $\var$ and transitions are consistent with assumptions and guarantees. At each step of an execution the environment selects values for the input variables in order to fulfill the assumptions and forcing the violation of a guarantee, while the controller responds by selecting a valuation of the output variables in order to satisfy the guarantees, thus taking the game to a new state. The controller synthesis problem is formalized into identifying a winning strategy for the controller in this game: a \emph{strategy} is a mapping from the history of past valuations in the game and the current input choice by the environment, to an output choice ensuring that the controller satisfy the guarantees. 
Formal definitions of games and strategies, and of the algorithm to compute controller strategies, are given in \cite{Bloem2012}.

If such a controller strategy does not exist, the GR(1) formula is said to be \emph{unrealizable}. In such a case there is a strategy for the environment that forces the violation of at least one guarantee \cite{Konighofer2009}. Such strategy is called a \emph{counterstrategy} and, symmetrically to strategies, maps histories of executions and the current state onto the next input choice by the environment. There are several formal definitions of counterstrategies \cite{Konighofer2009,Li2013,Cavezza2017}, all having in common its representation as a transition system whose states and/or transitions are labeled with valuations of variables. In our context this is the only aspect of interest, therefore we present here a simpler view of counterstrategies.

A \emph{counterstrategy} is a transition system $\counterstrategy = (Q_\counterstrategy, \delta_\counterstrategy, Q_0, \lambda_\counterstrategy)$, where $Q_\counterstrategy$ is a set of states, $\delta_\counterstrategy \subseteq Q_\counterstrategy \times Q_\counterstrategy$ is a set of transitions between states, $Q_0 \subseteq Q$ is a set of initial states, and $\lambda_\counterstrategy: Q \rightarrow 2^{\var \cup \mathcal{M}}$ is a labeling function for states. The labeling function assigns Boolean values to the system's variables in $\var$ and to a set of additional ``memory'' variables $\mathcal{M}$: these variables encode the history of visited states and affect the environment's next move from each state; these variables are added automatically by the algorithm in \cite{Konighofer2009} and are not supposed to appear anywhere in the assumptions or the guarantees.

A \emph{run} of the counterstrategy is any infinite sequence of states $q_1q_2\dots$ such that $q_1 \in Q_0$ and $(q_i,q_{i+1}) \in \delta_\counterstrategy$ for every $i \in \mathbb{N}$. Given a run, the associated \emph{play} is the infinite sequence of the labellings of its states $\pi = \lambda_\counterstrategy(q_1)\lambda_\counterstrategy(q_2)\dots$. By the definition of a counterstrategy, all of its plays satisfy the assumptions and violate at least one guarantee (in the sense of Section~\ref{sec:LTLGR1}). In the following we say that a counterstrategy $\counterstrategy$ satisfies the LTL formula $\phi$ ($\counterstrategy \models \phi$) if and only if all of its plays satisfy $\phi$. Therefore, a counterstrategy satisfies $\phi^\env$ and violates $\phi^\sys$.

\subsection{Counterstrategy-Guided Assumptions Refinement}
If a GR(1) specification $\phi^\env \rightarrow \phi^\sys$ is unrealizable, one way to fix it is to strengthen the existing assumptions so that the environment cannot force a guarantee violation under the new assumptions. A \emph{refinement} $\psi$ is a set of assumptions $\psi_1,\dots,\psi_k$ each of which is either an initial condition, an invariant, or a fairness condition. The problem of \emph{assumptions refinement} consists in finding one or more refinements $\psi$ such that $\phi^\env \land \psi \rightarrow \phi^\sys$ is a new GR(1) formula that is realizable. We call the solutions to the assumptions refinement problem \emph{sufficient refinements}.

Usually, when no other information on the environment but the assumptions $\phi^\env$ is input to the problem, an additional goal is finding a sufficient refinement that is the \emph{weakest} possible, in the sense of being the least constraining \cite{Li2011b,Cavezza2018,Seshia2015a}; this way the controller that can be synthesized from the refined specification is guaranteed to meet the specification in the widest possible set of environments. Moreover, since the new assumptions are to be understood and assessed by engineers, it is desirable that they be as concise as possible.

Typical assumptions refinement approaches are based on alternating between counterstrategy computations and assumption generation, and are called \emph{counterstrategy-guided} \cite{Li2011b, Li2013, Alur2013b, Cavezza2017}. Given an unrealizable specification with assumptions $\phi$, a counterstrategy $\counterstrategy_0$ is first computed by using the algorithm in \cite{Konighofer2009}, and one or more alternative assumptions $\psi_1, \dots, \psi_h$ inconsistent with $\counterstrategy_0$ are generated, using a bias as discussed in Section~\ref{sec:Motivating} Then, for each $\psi_i$, if $\phi \land \psi_i$ is still not sufficient, a new counterstrategy $\counterstrategy_i$ is generated, and again a set of assumptions $\psi_{i,1}, \dots \psi_{i,h'}$ inconsistent with $\counterstrategy_i$ is generated. Each of these assumptions is conjoined in turn to $\phi \land \psi_i$ and if the resulting specifications are still unrealizable, new counterstrategies are computed in the same fashion. The result is tree of refinements  that is explored in a breadth-first fashion, from smaller refinements to bigger ones, and whose leaves are solutions to the realizability problem \cite{Cavezza2017,Alur2013b,Li2011b,Maoz2019,Li2013}. We denote this approach as \emph{breadth-first search} (BFS).

The BFS approach ensures termination, since there are only finitely many non-equivalent logical conditions and the bias ensures only a small subset of them is actually explored. At every level of the refinement tree a finite number of assumptions is generated, and along a branch of the tree the assumptions are progressively strengthened by adding new conjuncts, until either they become inconsistent or a sufficient solution is formed \cite{Cavezza2017}. This however presents a problem. Suppose the search finds a sufficient refinement $\psi = \{\psi_1, \psi_2, \dots, \psi_k\}$; suppose also that a subset of these assumptions is sufficient, that is $\psi' \subset \psi$ is also sufficient to achieve realizability. This solution would not be checked during the incremental search, since there is no backtracking along the refinement tree.

In the following, with a slight abuse of notation, we will refer to a refinement $\psi$ both as a set of assumptions $\{\psi_1,\dots,\psi_k\}$ and as their conjunction $\psi_1 \land \dots \land \psi_k$.
%Hence, given a counterstrategy $\counterstrategy$, $\counterstrategy \models \psi$ can be both interpreted as $\counterstrategy$ satisfying each of the assumptions separately or their conjunction, the two statements being equivalent. As a final remark on notation, in the following
We will also refer to collections of \emph{sets} of counterstrategies $\mathcal{C} = \{C_1,\dots,C_k\}$ . We will denote their union as $\bigcup \mathcal{C} = \bigcup_{i=1}^k C_i$.


==> sections/conclusions.tex <==
\section{Conclusions}
In this paper we have proposed a new search method for assumptions refinement to solve the unrealizability problem for GR(1) specifications. We have provided a definition of redundancy of assumptions with respect to a set of counterstrategies and hence the concept of minimality of asssumptions. We have proposed an algorithm that returns minimal assumptions and integrated it in the classical counterstrategy-guided refinement loop. This provides a systematic way of trading off addition and replacement of assumptions when constructing refinements. The experiment shows that our approach achieves the goal of exploring a greater number of shorter specifications and finding shorter, non-redundant solutions.

==> sections/discussion.tex <==
\section{Discussion}

==> sections/improvements.tex <==
\section{Hybrid Refinement Generation}
\label{sec:Improvements}

While in BFS the explored candidate refinements keep increasing in length, when using minimization more iterations are needed before reaching longer refinements; this has two effects:
\begin{itemize}
	\item longer solutions require more execution time to be found;
	\item if the output of \textsc{ApplyBias} depends not only on the counterstrategy but also on the input $\phi^\env \land \psi$ (as is the case for interpolation, see \cite{Cavezza2017}), possibly an assumption needed to construct a solution can be computed only when an insufficient refinement of length $n$ is explored; reaching such partial refinement may require more time with minimization than with BFS.
\end{itemize}

\begin{example}
	In the AMBA04 case study (see Section~\ref{sec:Experiments}) a solution is $\psi = \always (\lnot \hready \rightarrow \next \hready)$, containing only one assumption. Interpolation does not compute this assumption until some partial refinement of length 3 is given as input to \textsc{ApplyBias}. This partial refinement is found by BFS in fewer iterations than Algorithm~\ref{alg:RefinementSearch}.
\end{example}

To soften this effect, our approach can be easily hybridized with BFS. It is sufficient to add to the queue the refinements explored by BFS together with the minimal refinements generated by Algorithm~\ref{alg:MinimalRefinement}, as done in lines 14-15.


==> sections/introduction-ijcai.tex <==
\section{Introduction}
In the last decade there has been a growing interest in automated synthesis from declarative specifications in Linear Temporal Logic (LTL) \cite{Camacho2018,DeGiacomo2015,Patrizi2013,Bloem2012}, with the goal of constructing correct-by-construction systems satisfying such logical properties. The approaches usually model the problem as finding a winning strategy in a two-player game, where an agent, the environment, tries to violate the specification, while the other, the controller, aims at satisfying it. Some approaches solve the game by reformulating it as a planning problem \cite{Camacho2018}, while others use purely symbolic, logic-based approaches, able to cope with large state spaces. This is the case of the subset of LTL called Generalized Reactivity 1 GR(1).

GR(1) specifications have an assume-guarantee form: they include a set of assumptions on the environment where the controller operates and only require a set of guarantees to be satisfied by the controller provided that the assumptions are satisfied too; no requirement is made when the environment violates its assumptions. In order for synthesis to be possible, the \emph{realizability} problem must be tackled first: that is, a sufficient set of assumptions must be provided so that no environment satisfying those assumptions can force a violation of the guarantees.

The goal of assumptions refinement is to perform a search on the set of possible assumptions in order to identify the ones sufficient for realizability. This search is expressed in the form of learning from counterexamples (counterexample-guided inductive synthesis, or CEGIS problem). In this framework, the search is guided by by \emph{counterstrategies}, environment strategies that force a guarantee violation \cite{Li2011b,Alur2013b,Cavezza2017}. The procedure is incremental: given an unrealizable specification, a counterstrategy is computed and a set of alternative assumptions that refine the initial ones is generated; if the new specification is still unrealizable, a new counterstrategy is again computed and new assumptions are generated to be added to the ones found in the previous step.

The problem with this incremental approach is that it is prone to generating solutions made up by large sets of assumptions. Such solutions are undesirable for three reasons:
\begin{itemize}
\item They are unreadable and thereby unintelligible by human engineers that need to assess whether such assumptions are reasonable about the environment;
\item The time to check realizability and compute counterstrategies grows linearly with the number of assumptions in the specification \cite{Bloem2012}; therefore, dealing with smaller intermediate refinements requires less time;
\item Redundant assumptions may be contained in the solution, that is a proper subset of the solution returned by the approach may also ensure realizability. Redundant solutions are undesirable since they drive the synthesis algorithm towards a specialized controller that works in a reduced set of environments.
\end{itemize}

We propose to use an approach that generates refinements by replacing redundant assumptions with new ones, rather than adding them. The approach uses model checking to verify whether an assumption $\psi$ generated from the counterstrategy $\mathcal{C}$ also eliminates one or more counterstrategies computed before $\mathcal{C}$; if so, one or more assumptions generated before $\psi$ are made redundant by $\psi$ and therefore replaced by it. We show how this approach generates shorter solutions that are less constraining than the ones generated by incremental addition.

==> sections/introduction.tex <==
\section{Introduction}
Reactive synthesis of controllers from declarative specifications is a well-known approach to obtain correct-by-construction systems \cite{Finkbeiner2016,DIppolito2010,Piterman2005,Bloem2012}. Specifications are expressed in the language of \emph{generalized reactivity of rank 1} (GR(1) for short), a subset of linear temporal logic (LTL) comprising invariants and fairness conditions. The promising successes of reactive synthesis have led to the annual synthesis competition SYNTCOMP \cite{SyntComp}, where synthesis tools compete on more than 500 benchmarks.

GR(1) specifications have an assume-guarantee form: they include a set of assumptions on the environmenst in which the controller operates and a set of guarantees to be satisfied by the controller in those environments. In order for synthesis to be possible, the \emph{realizability} problem must be tackled first: a specification is \emph{unrealizable} if there exists an adversarial environment that forces the violation of a guarantee for every controller. Assumptions refinement aims at identifying one or more sets of \emph{sufficient} assumptions, that are inconsistent with all such environments, in order to make the resulting specification realizable. This has two kinds of application in the literature. On one side, it is applied in contexts in which who produces the specification manually does not have a clear sense of the assumptions needed to ensure realizability \cite{Cimatti2008,Alur2013b,Maoz2019}. On the other hand, assumptions refinement has been used in the so-called human-in-the-loop controllers, as a way to identify one or more sets of assumptions that when violated trigger the controller to switch from automatic mode to human-controlled mode \cite{Li2013}.

Assumptions refinement is a search problem in an intractably large search space. To help direct the search towards a solution, state of the art approaches make use of \emph{counterstrategies}, characterizations of environment behaviors that force a guarantee violation \cite{Li2011b,Alur2013b,Cavezza2017}. The procedure is incremental: given an unrealizable specification, a counterstrategy $\counterstrategy$ is computed and a set of alternative assumptions $\psi$ inconsistent with $\counterstrategy$ is generated, where $\psi$ is a GR(1) formula; each $\psi$ is added in turn to the initial assumptions, and if the new specification is still unrealizable, a new counterstrategy $\counterstrategy'$ is then computed and a new assumption $\psi'$ is added to $\psi$, thus producing a new refinement $\psi \land \psi'$. An assumption inconsistent with a counterstrategy is also said to \emph{eliminate} such counterstrategy from the set of allowed environment behaviors.

The problem with this incremental approach is that it is prone to generating solutions made up by large sets of assumptions. When $\psi'$ is generated, it may be sufficient alone to also eliminate $\counterstrategy$; in this sense we say that $\psi$ becomes \emph{redundant} with respect to the counterstrategies $\counterstrategy$ and $\counterstrategy'$ once $\psi'$ is added. Therefore it would be desirable to replace $\psi'$ with $\psi$, rather than adding the former to the latter.

By eliminating such redundant refinements, two goals are achieved: (i) if $\psi'$ is a sufficient refinement to achieve realizability by itself, it is returned as a solution instead of the more restrictive $\psi \land \psi'$; this is desirable since the controller synthesized by using the former refinement is ensured to meet the guarantees in a wider set of environments; (ii) if $\psi'$ needs to be further refined, computing a counterstrategy and a further refinement from $\psi'$ requires in the worst case a shorter computation time than doing the same computation from $\psi \land \psi'$ (counterstrategy computation is linear in the number of assumptions, as for Theorem 3 in \cite{Bloem2012}); since shorter time is needed to elaborate each iteration of the search, more refinements can be explored in a fixed amount of time. In addition to these goals, the resulting refinements contain fewer assumptions, and engineers can therefore assess more easily whether those assumptions match the actual environment in which the controller is supposed to operate.

In this paper we formalize the notion of redundancy of assumptions with respect to the observed counterstrategies: given a refinement, an assumption in it is redundant if all the observed counterstrategies are already inconsistent with some of the other assumptions in the refinement; by eliminating all the redundant assumptions, we obtain what we call \emph{minimal} refinements. We provide a refinement minimization algorithm that provably removes any redundant assumption from a refinement; since this minimization can lead the search into infinite loops between the same refinements, we enhance the classical FIFO search criterion with duplicate checks. Moreover, since minimization can slow down the identification of a solution, we propose a hybrid refinement generation method that produces both non-minimal and minimal refinements. We finally show through experiments that by integrating the minimization algorithm in counterstrategy-guided approaches the search explores shorter refinements and produces shorter solutions, in particular some desirable solutions that would be missed otherwise. As a downside, when integrating minimization fewer solutions are found in the allotted time and the hybrid criterion is needed to mitigate this slowdown.

==> sections/modelchecking.tex <==
%!TEX root = ../main.tex
\section{Minimal Assumptions Sets}
A sufficient refinement is a set of assumptions such that any counterstrategy is inconsistent with their conjunction. The goal of counterstrategy-guided approaches is that of progressing towards a sufficient refinement by proposing at each step a candidate refinement that eliminates at least one new counterstrategy with respect to the previous candidate. If the new assumption removes one or more of the counterstrategies that were contained in the previous candidate, the corresponding assumptions generated at the previous steps may be redundant in order to form a solution. We formalize the notion of redundant assumption with respect to a set of counterstrategies.
\begin{definition}
	\label{def:RedundantAssumptions}
	Given a set of assumptions $\psi = \{\psi_1, \dots, \psi_n\}$ and a set of counterstrategies $C = \{\counterstrategy_1, \dots, \counterstrategy_{n}\}$, an assumption $\psi_i$ is \emph{redundant with respect to $\psi$ and $C$} if and only if for all $\counterstrategy_j \in C$, $\counterstrategy_j \not\models \bigwedge_{\psi_h \in \psi, h \ne i} \psi_h$.
\end{definition}

Notice that the definition of redundant assumption is well-formed: a counterstrategy $c \in C$ is inconsistent with a refinement $\psi = \psi_1 \land \dots \land \psi_n$ if and only if it is inconsistent with at least one $\psi_h$ alone. It is not the case that two or more assumptions are needed together to eliminate a counterstrategy, so, when a redundant assumption $\psi_j$ is removed from $\psi$, any other assumption $\psi_h \ne \psi_j$ still removes the same counterstrategies that were eliminated by $\psi$.

\begin{definition}
	\label{def:MinimalAssumptionsSet}
	A set of assumptions $\psi$ is said to be \emph{minimal} with respect to a set of counterstrategies $C$ if none of its assumptions is redundant (with respect to $\psi$ and $C$).
\end{definition}

In other words, an assumption $\psi_i$ in a refinement $\psi$ is redundant with respect to a set of counterstrategies $C$ if all the counterstrategies in $C$ are still eliminated when one removes $\psi_i$ from $\psi$. So, in order to construct a sufficient solution given some observed counterstrategies, $\psi_i$ may be safely deleted. A refinement not containing any redundant assumption is called minimal.

\section{Minimal Refinements Search}
\label{sec:MinimalRefinementsSearch}

In the followings we first describe  the minimization algorithm \textsc{MinimalRefinement}. Then we present the changes to the classical FIFO refinement algorithm \cite{Alur2013b,Cavezza2017} to avoid looping between duplicates.

\subsection{The function \textsc{MinimalRefinement}}
\label{sec:MinimalRefinement}

The core of our proposal is the function \textsc{MinimalRefinement}, shown in Algorithm~\ref{alg:MinimalRefinement}. This function adds a new assumption $\psi'$ to an insufficient refinement $\psi$ by ensuring the resulting refinement is minimal with respect to all the counterstrategies observed so far.

Specifically, suppose an unrealizable specification $\phi^\env \rightarrow \phi^\sys$ has been refined with the refinement $\psi = \{\psi_1,\dots,\psi_n\}$, which has been produced in an iterative process by eliminating the counterstrategies $C = \{\counterstrategy_1,\dots,\counterstrategy_n\}$. Suppose $\psi$ is not a sufficient refinement, therefore an additional counterstrategy $\counterstrategy'$ is computed, and a new assumption $\psi'$ is generated in order to eliminate $\counterstrategy'$. In general, each $\psi_i \in \psi$ and $\psi'$ may eliminate more than one counterstrategy in $C \cup \{\counterstrategy'\}$, and therefore by adding $\psi'$, some $\psi_i$ may become redundant with respect to $C \cup \{\counterstrategy'\}$.

In order to obtain minimality in the sense of Definition~\ref{def:MinimalAssumptionsSet}, the algorithm needs to know for each assumption which counterstrategies it eliminates. The relationship between the assumptions in a refinement and the eliminated counterstrategies can be pictured as a bipartite graph whose vertices are the elements $\psi_i \in \psi \cup \{\psi'\}$ and $\counterstrategy_j \in C \cup \{\counterstrategy'\}$, such that there is an edge $(\psi_i, \counterstrategy_j)$ if and only if $\counterstrategy_j \not\models \psi_i$.
\begin{figure}
	\centering
	\includegraphics[width=0.7\linewidth]{figs/bipartite_graph}
	\caption{Bipartite graph of assumptions and counterstrategies}
	\label{fig:bipartite_graph}
\end{figure}
\begin{example}
	An example is shown in Figure~\ref{fig:bipartite_graph}. In this example, $\psi_1$ eliminates $\counterstrategy_1$ only, $\psi_2$ removes $\counterstrategy_2$ and $\counterstrategy_3$, and $\psi_3$ removes $\counterstrategy_3$ and $\counterstrategy_4$. When adding $\psi'$, which removes $\counterstrategy_1$, $\counterstrategy_3$, $\counterstrategy_4$ and $\counterstrategy'$, the assumptions $\psi_1$ and $\psi_3$ become redundant.
\end{example}

Let the \emph{degree} of a vertex be the number of edges incident to that vertex. Then an assumption is redundant if and only if all the counterstrategies to which it is connected have a degree at least 2: indeed, even if such an assumption were eliminated, there would be another assumption eliminating all the counterstrategies connected to it. The algorithm then scans all the $\psi_i$'s and removes all redundant assumptions based on the degree of their connected counterstrategies; the resulting refinement will be minimal.
\begin{example}
	In Fig.~\ref{fig:bipartite_graph}, the addition of $\psi'$ makes $\psi_1$ and $\psi_3$ redundant: in fact, all the counterstrategies that are linked to them have degree of 2 or above. So, those two assumptions can be safely removed from the refinement.
\end{example}

\begin{algorithm}
	\caption{\textsc{MinimalRefinement} function}
	\label{alg:MinimalRefinement}
	\LinesNumbered
	\KwIn{$\psi = (\psi_1,\dots,\psi_k)$: insufficient refinement of cardinality $k$}
	\KwIn{$\mathcal{C}$: sequence of sets of eliminated counterstrategies with cardinality $k$}
	\KwIn{$\psi'$: assumption to be added to $\psi$}
	\KwIn{$\counterstrategy'$: a counterstrategy consistent with $\psi$ and eliminated by $\psi'$}
	\KwOut{$(\psi_\new, \mathcal{C}_\new)$: pair containing a minimal refinement $\psi \land \psi'$ and the corresponding set of eliminated counterstrategies}
	
	$C' \gets \{\counterstrategy'\}$\;	\label{alg:MinimalRefinement-line:StartComputeCPrime}	\label{alg:MinimalRefinement-line:InitCPrime}
	
	\ForEach{$\counterstrategy \in \bigcup \mathcal{C}$}{
		\If{$\counterstrategy \not\models \psi'$}{	\label{alg:MinimalRefinement-line:CSTest}
			$C' \gets C' \cup \{\counterstrategy\}$\;		\label{alg:MinimalRefinement-line:UpdateCPrime}
		}
	}
	\label{alg:MinimalRefinement-line:EndComputeCPrime}
	
	$\psi_\new \gets \psi$\;	\label{alg:MinimalRefinement-line:StartMinRefComputation} \label{alg:MinimalRefinement-line:StartInitMinRef}
	$\psi_\new$.append($\psi'$)\;
	$\mathcal{C}_\new \gets \mathcal{C}$\;
	$\mathcal{C}_\new$.append($C'$)\;		\label{alg:MinimalRefinement-line:EndInitMinRef}
	
	\ForEach{$\counterstrategy \in \bigcup \mathcal{C}_\new$}{	
		$\counterstrategy.degree$ = \textsc{CountSets}($\mathcal{C}_\new,\counterstrategy$)\;		\label{alg:MinimalRefinement-line:CountSets}
	}
	
	\For{$i = 1$ \KwTo $k$}{		\label{alg:MinimalRefinement-line:StartLoopMinRef}
		\If{$\forall \counterstrategy \in C_i \; \counterstrategy.degree \ge 2$}{	\label{alg:MinimalRefinement-line:RedundancyTest}
			$\psi_\new$.remove($\psi_i$)\;
			$\mathcal{C}_\new$.remove($C_i$)\;
			\ForEach{$\counterstrategy \in C_i$}{
				$\counterstrategy.degree \gets \counterstrategy.degree - 1$\;
			}
		}
	}		\label{alg:MinimalRefinement-line:EndLoopMinRef} \label{alg:MinimalRefinement-line:EndMinRefComputation}
	\Return{($\psi_\new,\mathcal{C}_\new$)}
	
\end{algorithm}

In order to construct the bipartite graph the algorithm needs to determine for each pair $(\psi_i, \counterstrategy_j)$ whether $\counterstrategy_j \models \psi_i$. This is a classical model checking problem, and can be solved with standard model checking algorithms \cite{Clarke1994}. However, in this setting there is no need to perform all the model checking operations for every pair $(\psi_i, c_j)$. \textsc{MinimalRefinement} is called as part of the loop in Algorithm~\ref{alg:RefinementSearch} (see Section~\ref{sec:SearchAlgorithm}): thereby at each call part of the bipartite graph is already constructed.

The inputs $\psi$ and $\mathcal{C}$ correspond to the bipartite graph produced in previous iterations. $\mathcal{C}$ is a collection of counterstrategy sets $C_i$ such that $\psi_i$ eliminates all the counterstrategies in $C_i$; that is, there is an edge between $\psi_i$ and each of the counterstrategies in $C_i$; $\psi'$ and $\counterstrategy'$ are the counterstrategy and the assumption produced in one iteration of the counterstrategy-guided approach (see Algorithm~\ref{alg:RefinementSearch}); hence, by hypothesis $\counterstrategy' \not\models \psi'$.

The function consists of two blocks. In the first one (lines \ref{alg:MinimalRefinement-line:StartComputeCPrime}-\ref{alg:MinimalRefinement-line:EndComputeCPrime}) the algorithm model-checks all the counterstrategies in $\bigcup \mathcal{C}$ against $\psi'$ and constructs the set $C' = \left\{\counterstrategy \in \bigcup \mathcal{C} \cup \{\counterstrategy'\} \:\middle|\: \counterstrategy \not\models \psi' \right\}$; by construction $\counterstrategy' \in C'$ (see line \ref{alg:MinimalRefinement-line:InitCPrime}).

The second block (lines~\ref{alg:MinimalRefinement-line:StartMinRefComputation}-\ref{alg:MinimalRefinement-line:EndMinRefComputation}) analyzes the bipartite graph and identifies the redundant assumptions: first, it builds the new refinement $\psi_\new = \psi \land \psi'$ to be minimized and the collection of counterstrategy sets $\mathcal{C}_\new$ by extending $\mathcal{C}$ accordingly with $C'$ (lines \ref{alg:MinimalRefinement-line:StartInitMinRef}-\ref{alg:MinimalRefinement-line:EndInitMinRef}). Then for every counterstrategy $\counterstrategy \in \bigcup \mathcal{C}_\new$ the function \textsc{CountSets} counts how many sets in $\mathcal{C}_\new$ contain $\counterstrategy$; this corresponds to the degree of the counterstrategy in the bipartite graph. Finally, lines~\ref{alg:MinimalRefinement-line:StartLoopMinRef}-\ref{alg:MinimalRefinement-line:EndLoopMinRef} remove any $\psi_i$ from $\psi_\new$ such that every counterstrategy in $C_i$ has degree greater or equal to 2.

\begin{example}
	Let us consider again the motivating example in Section~\ref{sec:Motivating}. In this case, $\psi_1 = \always\eventually \lnot \cl$ eliminates the first counterstrategy that has been generated, call it $\counterstrategy_1$; so $C_1 = \{\counterstrategy_1\}$ and $\mathcal{C} = \{C_1\}$. At the first call of \textsc{MinimalRefinement} the bipartite graph has a single assumption vertex and a single counterstrategy vertex; so, no minimization occurs.
	
	After the second counterstrategy is produced, $\psi_2 = \always (\lnot \val \rightarrow \next \lnot \cl)$ is generated. \textsc{MinimalRefinement} checks whether $\psi_2$ is also inconsistent with $\counterstrategy_1$ and finds that it does. So $C_2 = \{\counterstrategy_1,\counterstrategy_2\}$.
	
	Now $\counterstrategy_1$ has degree 2 and $\psi_1$ is only connected to $\counterstrategy_1$: therefore the algorithm finds that $\psi_1$ is redundant and it removes it when constructing the new refinement $\psi_\new$.
\end{example}

\subsection{Search Algorithm}
\label{sec:SearchAlgorithm}
State-of-the-art work on assumptions refinement \cite{Alur2013b,Cavezza2017} keep a FIFO queue of partial refinements: iteratively the first element of the queue is extracted, and if it is not sufficient a new set of alternative further refinements is generated and appended to the queue. If a refinement of size $n$ is extracted, the appended refinements have size $n+1$, and eventually no refinement of size $n$ remains in the queue. Therefore, even if the same refinements may appear in the queue more than once, each of them is explored a finite number of times.

In our context duplicate refinements are generated more frequently than in classical incremental approaches: testing for many duplicate refinements can delay finding a solution by a significant amount. The following example shows how minimization can lead to duplicates.
\begin{example}
	Suppose that $\psi_1 \land \psi'_2 $ is insufficient and the bias component of the algorithm (see Section~\ref{sec:Motivating}) generates the additional assumption $\psi_3$, which makes $\psi'_2$ redundant w.r.t. the observed counterstrategies. Suppose also that $\psi_1 \land \psi''_2$ is insufficient and again the bias generates $\psi_3$ that makes $\psi''_2$ insufficient; then $\psi_1 \land \psi_3$ is added twice to the queue of candidate refinements. All the further refinements being extensions of $\psi_1 \land \psi_3$ will also be explored twice, hence delaying reaching any solution. \IEEEQEDhere
\end{example}

One simple modification to the search would be keeping track of the refinements already explored and avoid re-expanding them. However, this may prevent progressing towards a solution. The following example serves to argue why also the counterstrategies eliminated by a refinement have to be considered when checking for duplicates.
\begin{example}
	Given an initial specification $\langle \phi^\env, \phi^\sys \rangle$, suppose $\psi_1 \land \psi_2 \land \psi_3$ is a solution to the realizability problem. The following table describes the steps of a FIFO refinement search given some bias.	
	\begin{center}
		\begin{tabular}{ccccc}
			& $(\psi,\bigcup \mathcal{C})$ & $\counterstrategy$ & $\Psi'$ & \textsc{MinRef}\\
			1	& $\varnothing$ & $\counterstrategy_1$		& $\psi_1$	& $\psi_1$ \\
			&				&							& $\psi_2$	& $\psi_2 $\\
			2	& $(\psi_1, \counterstrategy_1)$		& $\counterstrategy_2$		& $\psi_2$	& $\psi_2$ \\
			3	& $(\psi_2, \counterstrategy_1)$		& $\counterstrategy_3$		& $\psi_1$	&  $\psi_1$ \\
			4	& $(\psi_2, \counterstrategy_1, \counterstrategy_2)$		& $\counterstrategy_3$		& $\psi_1$  &  $\psi_2 \land \psi_1$ \\
		\end{tabular}
	\end{center}
	The column $(\psi,\bigcup \mathcal{C})$ contains the FIFO queue. At each search step, the first element in the queue is extracted, a counterstrategy $\counterstrategy$ is computed, and a set $\Psi'$ of alternative assumptions that eliminate $\counterstrategy$ is generated; the column \textsc{MinRef} shows the minimal refinement generated when adding the assumption in column $\Psi'$ to the refinement extracted from the queue given the observed counterstrategies in $\bigcup \mathcal{C}$ and $\counterstrategy$.
	
	At the beginning only the empty refinement is in the queue, the counterstrategy $\counterstrategy_1$ is produced and two assumptions $\psi_1$ and $\psi_2$ are generated, which are minimized and added to the queue in positions 2 and 3. Then in turn the refinement in position 2 is extracted from the queue, $\counterstrategy_2$ is computed, $\psi_2$ is generated by the bias and after minimizing $\psi_1 \land \psi_2$ w.r.t. the counterstrategies $\counterstrategy_1$ and $\counterstrategy_2$ only $\psi_2$ remains.
	
	Notice that $\psi_2$ is generated twice: once in iteration 1 as a standalone refinement, and once in iteration 2 as a result of the minimization procedure. Therefore it is popped twice from positions 3 and 4. At iteration 4, finally $\psi_2$ is not redundant and therefore it does not disappear after minimization. If the refinement $\psi_2$ were not explored twice, the refinement $\psi_2 \land \psi_1$ would not be added to the queue and the solution above could not be reached. The difference between the first and the second time $\psi_2$ is explored is in the counterstrategies it eliminates. \IEEEQEDhere
\end{example}

This suggests a different way of managing the queue and checking for duplicates, shown in Algorithm~\ref{alg:RefinementSearch}. As in the classical iterative search algorithms, the function \textsc{ComputeCounterstrategy} finds a counterstrategy to an unrealizable specification, and \textsc{ApplyBias} applies a bias to compute a set of alternative assumptions that eliminate that counterstrategy. However, instead of simply storing the refinements to explore, the queue $\candidateRefQueue$ contains both the refinements and the counterstrategies from which those were generated. An additional set $\exploredRefs$ is kept in memory to contain the pairs (refinement, counterstrategies) already explored. If the pair $(\psi, \mathcal{C})$ extracted from the queue is in $\exploredRefs$, then do not re-expand it. In order to avoid the complexity of checking equivalence between sets of counterstrategies, this comparison only takes into account the number of counterstrategies in $\bigcup \mathcal{C}$ (lines 6 and 19).

\begin{algorithm}
	\caption{\textsc{RefinementSearch} function}
	\label{alg:RefinementSearch}
	\SetAlgoLined
	\LinesNumbered
	\KwIn{$\phi^\env$: set of initial assumptions}
	\KwIn{$\phi^\sys$: set of guarantees}
	\KwOut{$\refs \subseteq \{\psi \:|\: \langle \phi^\env \land \psi, \phi^\sys \rangle \text{ is realizable}\}$}
	
	$\refs \gets \varnothing$\;
	$\candidateRefQueue \gets \{\varnothing\}$\;
	$\exploredRefs \gets \varnothing$\;
	\Repeat{$\candidateRefQueue = \varnothing$}{		\label{alg:ModifiedRefinement-line:QueueLoopStart}
		$(\psi, \mathcal{C}) \gets \candidateRefQueue$.dequeue()\;		\label{alg:ModifiedRefinement-line:PopFromQueue}
		\If{$\lnot (\psi, |\bigcup \mathcal{C}|) \in \exploredRefs$}{
			\uIf{\upshape not \textsc{IsRealizable}$\langle \phi^\env \land \psi, \phi^\sys\rangle$}{		\label{alg:ModifiedRefinement-line:RealizabilityTest}
				$\counterstrategy' \gets$ \textsc{ComputeCounterstrategy}($\phi^\env \land \psi, \phi^\sys$)\;		\label{alg:ModifiedRefinement-line:ComputeCounterstrategy}
				$\Psi' \gets$ \textsc{ApplyBias}($\counterstrategy', \phi^\env \land \psi, \phi^\sys$)\;		\label{alg:ModifiedRefinement-line:GenerateAlternativeAssumptions}
				\ForEach{$\psi' \in \Psi'$}{
					$(\psi_\new, \mathcal{C}_\new) \gets$ \textsc{MinimalRefinement}($\psi, \mathcal{C}, \psi', \counterstrategy'$)\;		\label{alg:ModifiedRefinement-line:CallMinimalRefinement}
					$\candidateRefQueue$.enqueue($(\psi_\new, \mathcal{C}_\new)$)\;
					\uIf{hybrid}{
						$C' \gets $ last set in $\mathcal{C}_\new$\;
						$\candidateRefQueue$.enqueue($(\psi \cup \{\psi'\}, \mathcal{C} \cup \{C'\})$)\;
					}
				}
			}
			\uElseIf{\textsc{IsSatisfiable}($\phi^\env \land \psi$)}{		\label{alg:ModifiedRefinement-line:SatCheck}
				$\refs$.append($\psi$)\;
			}
			$\exploredRefs$.append($(\psi, |\bigcup \mathcal{C}|)$)\;
		}
	}		\label{alg:ModifiedRefinement-line:QueueLoopEnd}
	\Return{$\refs$}
\end{algorithm}

==> sections/motivation.tex <==
\section{Motivating Example}
\label{sec:Motivating}

As a running example, consider the request-grant protocol described in \cite{Alur2013b}.  This protocol consists of two input variables, $\req$ and $\cl$, that the environment uses respectively to request access to some resource and to clear that resource; and two output variables, $\gr$ and $\val$, which respectively grant access to the resource and signal whether it is in a valid state.

GR(1) specifications extend the classical Boolean logic with the operators $\always$ (``always''), $\eventually$ (``eventually''), and $\next$ (``next''); these are formalized in Section~\ref{sec:Background}.
The initial assumption $\phi^\env = \always\eventually \lnot \req$ ensures that the environment does not request access continuously. The guarantees
$\phi^\sys_1 = \always(\req \rightarrow \next\eventually \gr)$%
\footnote{Notice that this guarantee does not strictly abide by the GR(1) syntax. However, the work in \cite{Maoz2015a} shows that such formulae can be converted to pure GR(1) via the addition of auxiliary variables},
$\phi^\sys_2 = \always((\cl \lor \gr) \rightarrow \next \lnot \gr)$,
$\phi^\sys_3 = \always(\cl \rightarrow \lnot \val)$,
$\phi^\sys_4 = \always\eventually(\gr \land \val)$
represent some common requirements of request-grant protocols: that a request be eventually followed by a grant; that whenever a clear or a grant is active at some time step, the grant be unset at the following step; that whenever a clear is issued, the valid flag be unset; and that the environment can access valid data infinitely many times.

This specification is unrealizable: indeed an environment that keeps the $\cl$ to $\true$ prevents any controller from fulfilling at the same time the guarantees $\phi^\sys_3$ and $\phi^\sys_4$ (Fig.~\ref{fig:counterstrategyExample2}).
\begin{figure}
	\centering
	\includegraphics[width=0.7\linewidth]{figs/counterstrategyExample2}
	\caption{Simplified counterstrategy for the request-grant example. The output variables and the memory variables are omitted for clarity}
	\label{fig:counterstrategyExample2}
\end{figure}

Assumptions refinement has to look into an infinite space of possible assumptions (or doubly exponentially large in the number of variables, if logical equivalence is taken into account) in order to find a solution. For this reason, a criterion is always employed to decide which subset of formulae to generate \cite{Li2011b,Alur2013b,Cavezza2017}: we call such criterion \emph{bias}, as it is in fact an inductive bias imposed on the solution space. This bias, however, may prevent the search from reaching a desirable solution.

Consider, e.g., the interpolation mechanism of \cite{Cavezza2017}. After a counterstrategy is computed (see Fig.~\ref{fig:counterstrategyExample2}), the first assumption returned via interpolation is $\psi = \always\eventually \lnot \cl$, which forces the environment to set $\cl$ to $\false$ infinitely many times. This is still not sufficient to achieve realizability, since an environment can force the violation of the guarantees by setting $\cl$ to $\true$ at any time following a time step where $\val$ is $\false$; this way $\phi^\sys_4$ can never be satisfied as $\gr$ and $\val$ are never satisfied together. Therefore a new counterstrategy is computed and $\psi_2 = \always (\lnot \val \rightarrow \next \lnot \cl)$ is generated to eliminate this counterstrategy.

The refinement $\psi = \psi_1 \land \psi_2$ is sufficient, and is returned as a solution by the approach in \cite{Cavezza2017}; however even the assumption $\psi_2$ alone would be, and $\psi_1$ is therefore redundant. If $\psi_2$ were to replace $\psi_1$ instead of being conjoined to it, the resulting solution would provide a weaker constraint on the environment.

In general, the search algorithm has to trade off between replacements and concatenations of assumptions when looking for a solution: concatenating assumptions typically leads to more constrained environments where realizability can be more easily achieved; on the other hand replacements generate less constraining refinements that can yield more desirable solutions. This paper presents a heuristic criterion to balance between concatenations and replacements.

==> sections/related.tex <==
\section{Related Work}
\label{sec:Related}
As pointed out above, our work follows the lines of \cite{Li2011b,Alur2013b,Cavezza2017} in using counterstrategies for generating assumptions. However, unlike these works, that focus on proposing on defining language biases in generating new assumptions from single counterstrategies (that is, on the function \textsc{ApplyBias} in Algorithm~\ref{alg:RefinementSearch}), our work focuses on a novel search strategy, based on mutating the explored refinements rather than strengthening them. Our strategy to generate new refinements to explore, instead of using local information on the last counterstrategy observed, uses information at the level of an entire refinement, that is all the counterstrategies eliminated by that refinement. As a matter for future work, the next level will be using global information about the entire set of counterstrategies observed during the search.

The work in \cite{Kuvent2017} defines a more efficient alternative to counterstrategies, namely Justice Violation Transition Systems (JVTSes), an abstraction of counterstrategies where cycle states and transient states are merged into macro-states. A work on refining assumptions by using JVTSes is soon to be published \cite{Maoz2019}. This approach affects the functions \textsc{ComputeCounterstrategy} and \textsc{ApplyBias} from Algorithm~\ref{alg:RefinementSearch}. However, since our \textsc{MinimalRefinement} procedure treats counterstrategies as abstract objects, only exploiting their satisfaction relation with assumptions, it can be seamlessly applied to JVTSes instead; the only point to be careful of is defining the satisfaction of an LTL formula by a JVTS, which represents a set of counterstrategies rather than a single one.

The problem of reactive synthesis from logical specifications was formalized by Church \cite{Church1962} and found to require doubly exponential time in the length of the specification for LTL (see \cite{Finkbeiner2016} for a review of synthesis algorithms for various logics). GR(1) has received particular attention in the last years due to the discovery of the linear-time algorithm in \cite{Piterman2005,Bloem2012}. This algorithm is \emph{symbolic}: it represents game and strategy states directly through the valuations of the variables in $\var$, and sets of states as Boolean formulae over these variables; the use of efficient data structures like Binary Decision Diagrams (BDDs, \cite{Meinel1998}) drastically reduces the average space requirements allowing to represent entire state spaces in a compact form. A different thread of research focuses on different subsets of LTL \cite{Camacho2018,DeGiacomo2015,Patrizi2013} and the synthesis problem is reduced to planning; however, these approaches use explicit-state representations, and in order to counter the state explosion problem they define bounded-time versions of realizability or finite-time versions of LTL. A similar remark on the trade off between using BDDs and completeness with respect to LTL is elicited in Section 4.1.1 of \cite{Kupferman2006}.

The definition of minimal sets of assumptions is inspired by the problem of minimum set cover (treated in its general form in Chapter 2 of \cite{Vazirani2003a}, and in a more specific form closer to our setting in \cite{Bazgan2005}). Given a set of elements $C$ and a collection $S$ of subsets of $C$, the minimum set cover is a subcollection of subsets $S' \subseteq S$ such that $\bigcup S' = C$ and $S'$ contains the least number of subsets needed to cover $C$. Notice that our problem of finding minimal refinements is a relaxation of this NP-hard problem, as in our formulation we are not interested in minimizing the number of subsets; rather, our notion of minimality corresponds to the notion of non-redundancy in \cite{Bazgan2005}. Accordingly, Algorithm~\ref{alg:MinimalRefinement} is a simplification of the greedy algorithm \textsc{SCGreedy} described in \cite{Bazgan2005}: our algorithm does not select the assumption that removes the most counterstrategies at each step (as in line 2 of \textsc{SCGreedy}). This step could be easily included in our approach, however in our case studies would not produce a sensible improvement, since all explored nodes are already of length at most 3 (Section~\ref{sec:Experiments}).

Redundancy and minimization in logical formulae has already been studied extensively, such as in \cite{Gottlob1993,Guthmann2017,Liberatore2005,Nguyen2014a}. The notion of redundancy we present here is substantially different from the one in the literature. Redundancy in logic is typically related to implication and entailment: a formula or a clause is redundant if another one in the knowledge base entails it. In our case, redundancy is defined with respect to the goal of eliminating a sample of counterstrategies: one assumption may not be entailed by any other in a refinement and still be redundant if all the observed counterstrategies are eliminated by the other assumptions in the refinement.
